The Unlocking Spell on Base LLMs: Rethinking Alignment via In-Context Learning

The alignment tuning process of large language models (LLMs) typically involves instruction learning through supervised fine-tuning (SFT) and preference tuning via reinforcement learning from human feedback (RLHF). A recent study, LIMA (Zhou et al. 2023), shows that using merely 1K examples for SFT can achieve significant alignment performance as well, suggesting that the effect of alignment tuning might be "superficial." This raises questions about how exactly the alignment tuning transforms a base LLM. We analyze the effect of alignment tuning by examining the token distribution shift between base LLMs and their aligned counterpart. Our findings reveal that base LLMs and their alignment-tuned versions perform nearly identically in decoding on the majority of token positions. Most distribution shifts occur with stylistic tokens. These direct evidence strongly supports the Superficial Alignment Hypothesis suggested by LIMA. Based on these findings, we rethink the alignment of LLMs by posing the research question: how effectively can we align base LLMs without SFT or RLHF? To address this, we introduce a simple, tuning-free alignment method, URIAL. URIAL achieves effective alignment purely through in-context learning (ICL) with base LLMs, requiring as few as three constant stylistic examples and a system prompt. We conduct a fine-grained and interpretable evaluation on a diverse set of examples, named JUST-EVAL-INSTRUCT. Results demonstrate that base LLMs with URIAL can match or even surpass the performance of LLMs aligned with SFT or SFT+RLHF. We show that the gap between tuning-free and tuning-based alignment methods can be significantly reduced through strategic prompting and ICL. Our findings on the superficial nature of alignment tuning and results with URIAL suggest that deeper analysis and theoretical understanding of alignment is crucial to future LLM research.

==> 5_analysis.tex <==
 

==> 7_limitation.tex <==
% \section{Limitations}


==> tab_main.tex <==
\begin{table*}[t]
\vspace{-3em}
\hspace{-0.5em}
% \centering
\scalebox{0.9}{
 
\begin{tabular}{@{}cccccccc@{}}
% \toprule
 \textbf{Method} &  {\small \hspace{-1em}\faInfoCircle\textbf{Relevant}} &  {\small \hspace{-1em}\faIndent\textbf{Coherent}} &   {\small {\faCheckSquare[regular]}\textbf{Factual}} &   {\small \faCommentMedical\textbf{Deep}} &   {\small \hspace{-1em}\faLaughBeam[regular]\textbf{Engaging}} &   {\small \hspace{-1em}\faShieldVirus\textbf{Safety}} &   {\small \textbf{Overall}} \\
\midrule
 \rowcolor[gray]{0.95} \textit{Untuned 7B} $\downarrow$ & \multicolumn{6}{c}{$\ge$ \textbf{\texttt{Llama-2-7b-chat} (SFT+RLHF)}} &  \vspace{0.3em}  \\
 % Llama-2-7b-chat-hf $\ge$ vicuna-7b-v1.5     &        91.2 &        89.4 &         92.6 &    78.4 &         90.6 &    100   &     90.37 &   249.466 \\
 % K=3long (7b) $\ge$ vicuna-7b-v1.5           &        92.4 &        87.4 &         93.2 &    78.8 &         89.6 &     99.2 &     90.1  &   170.348 \\
 Templ. Prompt            & 52.0$\supseteq$5.6  & 34.2$\supseteq$5.8  & 61.2$\supseteq$5.8   & 27.8$\supseteq$11.2 & 24.8$\supseteq$3.8   & 88.2$\supseteq$0.0  &     48.1 \\
 Basic ICL (K=3)      & 59.0$\supseteq$5.2  & 36.2$\supseteq$6.6  & 63.6$\supseteq$5.4   & 24.2$\supseteq$8.0  & 23.2$\supseteq$3.8   & 89.8$\supseteq$0.2  &     49.3  \\
 Retrieved (K=3)      & 78.2$\supseteq$9.2  & 73.4$\supseteq$10.2 & 86.0$\supseteq$7.6   & 61.0$\supseteq$22.6 & 61.2$\supseteq$7.0   & 92.0$\supseteq$0.4  &     75.3   \\
 \hdashline[2pt/2pt]  \vspace{-0.7em} \\  
 \methodname{} (K=1)      & 83.2$\supseteq$10.0 & 79.2$\supseteq$9.8  & 86.8$\supseteq$8.4   & 63.6$\supseteq$23.6 & 70.0$\supseteq$10.0  & 93.4$\supseteq$0.4  &     79.4  \\
 \methodname{} (K=2)       & 85.6$\supseteq$11.4 & 82.8$\supseteq$13.4 & 86.8$\supseteq$8.0   & 68.4$\supseteq$25.2 & 73.6$\supseteq$12.0  & 92.6$\supseteq$0.0  &     81.6   \\ 
 \methodname{} (K=3)       & \textbf{88.2}$\supseteq$12.2 & 81.8$\supseteq$13.2 & 88.0$\supseteq$8.2   & 69.2$\supseteq$27.4 & 75.4$\supseteq$12.8  & 93.8$\supseteq$0.2  &     82.7   \\ 
\methodname{} (K=3;RA) & 87.6$\supseteq$14.4 & \textbf{87.2}$\supseteq$10.2 & \textbf{89.2}$\supseteq$9.2   & \textbf{73.2}$\supseteq$28.8 & \textbf{85.8}$\supseteq$15.2  & \textbf{94.2}$\supseteq$0.0  &     \textbf{86.2}  \\

 \midrule 
 \rowcolor[gray]{0.95} \textit{7B LLMs} $\downarrow$ & \multicolumn{6}{c}{$\ge$ \textbf{\texttt{Vicuna-v1.5-7b} (SFT only)}} &  \vspace{0.3em} \\
 SFT+RLHF  & 91.2$\supseteq$9.6  & \textbf{89.4}$\supseteq$12.8 & 92.6$\supseteq$9.0 & 78.4$\supseteq$24.4 & 90.6$\supseteq$19.6 & \textbf{100.0}$\supseteq$5.8 &      90.4 \\
 \methodname{} (K=3)       & 92.4$\supseteq$7.2  & 87.4$\supseteq$8.8  & 93.2$\supseteq$8.2 & 78.8$\supseteq$23.6 & 89.6$\supseteq$7.8  & 99.2$\supseteq$0.2  &      90.1 \\
 \methodname{} (K=3;RA) & \textbf{95.0}$\supseteq$9.4  & 87.0$\supseteq$15.4 & \textbf{96.0}$\supseteq$8.6 & \textbf{81.2}$\supseteq$30.4 & \textbf{93.2}$\supseteq$27.4 & 99.6$\supseteq$0.4  &      92.0   \\
 \midrule
\rowcolor[gray]{0.95} \textit{70B LLMs} $\downarrow$ &  \multicolumn{6}{c}{$\ge$ \textbf{OpenAI's \texttt{gpt-3.5-turbo}}} & \vspace{0.3em}\\
 SFT+RLHF & 91.8$\supseteq$7.2  & \textbf{91.8}$\supseteq$5.2  & 94.4$\supseteq$5.6 & \textbf{82.2}$\supseteq$13.8 & 90.8$\supseteq$9.2  & \textbf{99.8}$\supseteq$3.4  &      \textbf{91.8} \\
 \methodname{}(K=3)    & 92.8$\supseteq$3.4  & 89.4$\supseteq$4.4  & 96.4$\supseteq$4.2 & 75.8$\supseteq$10.8 & 90.6$\supseteq$4.8  & 99.6$\supseteq$0.0  &      90.8 \\
 \methodname{}(K=3;RA) & \textbf{94.8}$\supseteq$3.4  & 90.8$\supseteq$8.8  & \textbf{97.4}$\supseteq$4.4 & 76.8$\supseteq$15.0 & \textbf{91.4}$\supseteq$15.0 & \textbf{99.8}$\supseteq$0.8  &      \textbf{91.8} \\
 % K=3long (70b)            &        92.8 &        89.4 &         96.4 &    75.8 &         90.6 &     99.6 &     90.77 &   161.11  \\
 % llama-2-chat (70b) $\ge$ gpt-4              &        91.2 &        93.6 &         94.6 &    82.4 &         92.2 &     99.8 &     92.3  &   254.228 \\
 % llama-2-chat (70b) $\ge$ gpt-4-0314         &        90   &        91.6 &         93   &    80.8 &         90.8 &    100   &     91.03 &   254.228 \\
\bottomrule
\end{tabular}
}
\caption{\small 
\textbf{Multi-aspect pairwise evaluation of different alignment methods.} \methodname{} methods utilize K curated in-context examples to align untuned LLMs and incorporate an additional contrastive alignment (CA) step. The figures in the ``X$\supseteq$Y'' format indicate that method A is \textit{better than or equally good as} method B in $X\%$ of the examples, and A is strictly superior to B in $Y\%$ of the examples.
\vspace{-1em}
}
\label{tab:pair}
\end{table*}






==> tab_main_backup.tex <==
\begin{table*}[t]
\vspace{-1.5em}
\hspace{-0.5em}
% \centering
\scalebox{0.9}{
 
\begin{tabular}{@{}cccccccc@{}}
% \toprule
 \textbf{Method} &  {\small \hspace{-1em}\faInfoCircle\textbf{Relevant}} &  {\small \hspace{-1em}\faIndent\textbf{Coherent}} &   {\small {\faCheckSquare[regular]}\textbf{Factual}} &   {\small \faCommentMedical\textbf{Deep}} &   {\small \hspace{-1em}\faLaughBeam[regular]\textbf{Engaging}} &   {\small \hspace{-1em}\faShieldVirus\textbf{Safety}} &   {\small \textbf{Overall}} \\
\midrule
 \rowcolor[gray]{0.95} \textit{Untuned 7B} $\downarrow$ & \multicolumn{6}{c}{$\ge$ \textbf{\texttt{Llama-2-7b-chat} (SFT+RLHF)}} &  \vspace{0.3em}  \\
 % Llama-2-7b-chat-hf $\ge$ vicuna-7b-v1.5     &        91.2 &        89.4 &         92.6 &    78.4 &         90.6 &    100   &     90.37 &   249.466 \\
 % K=3long (7b) $\ge$ vicuna-7b-v1.5           &        92.4 &        87.4 &         93.2 &    78.8 &         89.6 &     99.2 &     90.1  &   170.348 \\
 Templ. Prompt            & 52.0$\supseteq$5.6  & 34.2$\supseteq$5.8  & 61.2$\supseteq$5.8   & 27.8$\supseteq$11.2 & 24.8$\supseteq$3.8   & 88.2$\supseteq$0.0  &     48.1 \\
 Basic ICL (K=3)      & 59.0$\supseteq$5.2  & 36.2$\supseteq$6.6  & 63.6$\supseteq$5.4   & 24.2$\supseteq$8.0  & 23.2$\supseteq$3.8   & 89.8$\supseteq$0.2  &     49.3  \\
 Retrieved (K=3)      & 78.2$\supseteq$9.2  & 73.4$\supseteq$10.2 & 86.0$\supseteq$7.6   & 61.0$\supseteq$22.6 & 61.2$\supseteq$7.0   & 92.0$\supseteq$0.4  &     75.3   \\
 
 \methodname{} (K=1)      & 83.2$\supseteq$10.0 & 79.2$\supseteq$9.8  & 86.8$\supseteq$8.4   & 63.6$\supseteq$23.6 & 70.0$\supseteq$10.0  & 93.4$\supseteq$0.4  &     79.4  \\
 \methodname{} (K=2)       & 85.6$\supseteq$11.4 & 82.8$\supseteq$13.4 & 86.8$\supseteq$8.0   & 68.4$\supseteq$25.2 & 73.6$\supseteq$12.0  & 92.6$\supseteq$0.0  &     81.6   \\ 
 \methodname{} (K=3)       & 88.2$\supseteq$12.2 & 81.8$\supseteq$13.2 & 88.0$\supseteq$8.2   & 69.2$\supseteq$27.4 & 75.4$\supseteq$12.8  & 93.8$\supseteq$0.2  &     82.7   \\ 
\methodname{} (K=3;RA) & 87.6$\supseteq$14.4 & 87.2$\supseteq$10.2 & 89.2$\supseteq$9.2   & 73.2$\supseteq$28.8 & 85.8$\supseteq$15.2  & 94.2$\supseteq$0.0  &     86.2   \\

 \midrule 
 \rowcolor[gray]{0.95} \textit{7B LLMs} $\downarrow$ & \multicolumn{6}{c}{$\ge$ \textbf{\texttt{Vicuna-v1.5-7b} (SFT only)}} &  \vspace{0.3em} \\
 SFT+RLHF  & 91.2$\supseteq$9.6  & 89.4$\supseteq$12.8 & 92.6$\supseteq$9.0 & 78.4$\supseteq$24.4 & 90.6$\supseteq$19.6 & 100.0$\supseteq$5.8 &      90.4 \\
 \methodname{} (K=3)       & 92.4$\supseteq$7.2  & 87.4$\supseteq$8.8  & 93.2$\supseteq$8.2 & 78.8$\supseteq$23.6 & 89.6$\supseteq$7.8  & 99.2$\supseteq$0.2  &      90.1 \\
 \methodname{} (K=3;RA) & 95.0$\supseteq$9.4  & 87.0$\supseteq$15.4 & 96.0$\supseteq$8.6 & 81.2$\supseteq$30.4 & 93.2$\supseteq$27.4 & 99.6$\supseteq$0.4  &      92.0   \\
 \midrule
\rowcolor[gray]{0.95} \textit{70B LLMs} $\downarrow$ &  \multicolumn{6}{c}{$\ge$ \textbf{OpenAI's \texttt{gpt-3.5-turbo}}} & \vspace{0.3em}\\
 SFT+RLHF & 91.8$\supseteq$7.2  & 91.8$\supseteq$5.2  & 94.4$\supseteq$5.6 & 82.2$\supseteq$13.8 & 90.8$\supseteq$9.2  & 99.8$\supseteq$3.4  &      91.8 \\
 \methodname{}(K=3)    & 92.8$\supseteq$3.4  & 89.4$\supseteq$4.4  & 96.4$\supseteq$4.2 & 75.8$\supseteq$10.8 & 90.6$\supseteq$4.8  & 99.6$\supseteq$0.0  &      90.8 \\
 \methodname{}(K=3;RA) & 94.8$\supseteq$3.4  & 90.8$\supseteq$8.8  & 97.4$\supseteq$4.4 & 76.8$\supseteq$15.0 & 91.4$\supseteq$15.0 & 99.8$\supseteq$0.8  &      91.8 \\
 % K=3long (70b)            &        92.8 &        89.4 &         96.4 &    75.8 &         90.6 &     99.6 &     90.77 &   161.11  \\
 % llama-2-chat (70b) $\ge$ gpt-4              &        91.2 &        93.6 &         94.6 &    82.4 &         92.2 &     99.8 &     92.3  &   254.228 \\
 % llama-2-chat (70b) $\ge$ gpt-4-0314         &        90   &        91.6 &         93   &    80.8 &         90.8 &    100   &     91.03 &   254.228 \\
\bottomrule
\end{tabular}
}
\caption{\small 
\textbf{Multi-aspect pairwise evaluation of different alignment methods.} \methodname{} methods utilize K curated in-context examples to align untuned LLMs and incorporate an additional contrastive alignment (CA) step. The figures in the ``X$\supseteq$Y'' format indicate that method A is \textit{better than or equally good as} method B in $X\%$ of the examples, and A is strictly superior to B in $Y\%$ of the examples.
\vspace{-1em}
}
\label{tab:pair}
\end{table*}






==> tab_score.tex <==
\begin{table*}[t]
\vspace{-2.5em}
\hspace{-0.5em}
\centering
\scalebox{0.9}{
 
\begin{tabular}{@{}cccccccc@{}}
% \toprule
 \textbf{7B/ 70B / GPTs} &  {\small \hspace{-1em}\faInfoCircle\textbf{Relevant}} &  {\small \hspace{-1em}\faIndent\textbf{Coherent}} &   {\small {\faCheckSquare[regular]}\textbf{Factual}} &   {\small \faCommentMedical\textbf{Deep}} &   {\small \hspace{-1em}\faLaughBeam[regular]\textbf{Engaging}} &   {\small \hspace{-1em}\faShieldVirus\textbf{Safety}} &   {\small \textbf{Overall}} \\
\midrule
 \rowcolor[gray]{0.9} Templated Prompt       &        6.10  &        7.30  &         6.68 &    5.25 &         6.15 &     9.66 &      6.86 \\
 Vicuna-v1.5 (\textbf{SFT})      &        \textbf{8.73} &        \underline{9.45} &         \underline{8.57} &    \textbf{7.87} &         8.31 &     \textbf{9.99} &      \textbf{8.82} \\
 Llama2-Chat (+\textbf{RLHF})     &        8.31 &        \textbf{9.56} &        \textbf{8.73} &    \underline{7.83} &         \textbf{8.50}  &     \textbf{9.99} &      \textbf{8.82} \\
 \textbf{\methodname{}} (K=3)        &        \underline{8.32} &        9.32 &         8.28 &    7.54 &         8.17 &     9.96 &      8.60  \\
 \textbf{\methodname{}} (K=3; RA)  &        8.18 &        9.29 &         8.33 &    7.73 &         \underline{8.34} &     9.96 &      8.64 \\ \midrule
 Llama2-70b-Chat     &        8.90  &        \textbf{9.75} &         \underline{9.11} &    \textbf{8.38} &         \underline{8.65} &     \textbf{9.99} &     \underline{9.13} \\
 \textbf{\methodname{}} (K=3)-70B       &        \textbf{9.24} &        9.57 &         9.06 &    8.25 &         8.48 &     9.93 &      9.09 \\
 \textbf{\methodname{}} (K=3; RA)-70B &        \underline{9.12} &        \underline{9.72} &        \textbf{ 9.21} &    \underline{8.31} &         \textbf{8.72} &     \underline{9.96} &      \textbf{9.17} \\ \midrule
 OpenAI ChatGPT             &        \underline{9.70}  &        \underline{9.95} &         \underline{9.66} &    \underline{8.90}  &        \underline{8.76} &    \textbf{ 9.99} &      \underline{9.49} \\
  OpenAI GPT4          &        \textbf{9.80}  &        \textbf{9.96} &         \textbf{9.71} &    \textbf{8.96} &         \textbf{8.79} &     \underline{9.95} &      \textbf{9.53} \\
 % gpt4                &     9.7     &     9.954   &      9.662   & 8.794   &      8.706   &  9.96    &     9.463 \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Multi-aspect scoring evaluation of different alignment methods.} \methodname{} methods use K stylistic examples to align untuned LLMs and add an optional contrastive alignment (CA) step. \vspace{-1.5em}}   
\label{tab:score}
\end{table*}
